Autoregressive Queries for Adaptive Tracking with Spatio-TemporalTransformers

The rich spatio-temporal information is crucial to capture the complicated target appearance variations in visual tracking. However, most top-performing tracking algorithms rely on many hand-crafted components for spatio-temporal information aggregation. Consequently, the spatio-temporal information is far away from being fully explored. To alleviate this issue, we propose an adaptive tracker with spatio-temporal transformers (named AQATrack), which adopts simple autoregressive queries to effectively learn spatio-temporal information without many hand-designed components. Firstly, we introduce a set of learnable and autoregressive queries to capture the instantaneous target appearance changes in a sliding window fashion. Then, we design a novel attention mechanism for the interaction of existing queries to generate a new query in current frame. Finally, based on the initial target template and learnt autoregressive queries, a spatio-temporal information fusion module (STM) is designed for spatiotemporal formation aggregation to locate a target object. Benefiting from the STM, we can effectively combine the static appearance and instantaneous changes to guide robust tracking. Extensive experiments show that our method significantly improves the tracker's performance on six popular tracking benchmarks: LaSOT, LaSOText, TrackingNet, GOT-10k, TNL2K, and UAV123.

==> sec/figs/fig4.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{4-.pdf}
    \caption{Illustration of the STM(spatial and temporal fusion operation module).}
    \label{fig:4-}
\end{figure} 

==> sec/figs/fig5.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{5-.pdf}
    \caption{Illustration of the self-attention or cue attention used in the temporal decoder.}
    \label{fig:5-}
\end{figure} 

==> sec/table/ca-attention.tex <==
\begin{table}[t]
    \caption{The effect of the clue attention(CA).}
    \centering
    % \resizebox{\linewidth}{!}{
        \fontsize{9}{11}\selectfont
        \begin{tabular}{c|ccc}
        \toprule
          & AUC & P$_{norm}$ &P\\
         \midrule
         self-attention & 70.7 & 80.9 & 77.8 \\ %使用的是self-attention，需要切片
         clue attention &\textbf{71.4} & \textbf{81.9} & \textbf{78.6} \\
        \bottomrule 
        \end{tabular}
        % }
    
    \label{tab:ca-attention}
\end{table} 

